Too Many Options: A Survey of ABE Libraries for Developers

Attribute-based encryption (ABE) comprises a set of one-to-many encryption schemes that allow the encryption and decryption of data by associating it with access policies and attributes. Therefore, it is an asymmetric encryption scheme, and its computational requirements limit its deployment in IoT devices. There are different types of ABE and many schemes within each type. However, there is no consensus on the default library for ABE, and those that exist implement different schemes. Developers, therefore, face the challenge of balancing efficiency and security by choosing the suitable library for their projects. This paper studies eleven ABE libraries, analyzing their main features, the mathematical libraries used, and the ABE schemes they provide. The paper also presents an experimental analysis of the four libraries which are still maintained and identifies some of the insecure ABE schemes they implement. In this experimental analysis, we implement the schemes offered by these libraries, measuring their execution times on architectures with different capabilities, i.e., ARMv6 and ARMv8. The experiments provide developers with the necessary information to choose the most suitable library for their projects, according to objective and well-defined criteria.

==> Docs/recortes.tex <==
% \subsubsection{RECICLAR LW11}

% \added{LW11~\cite{lewko2011decentralizin} was one of the first decentralized \ac{CP-ABE} schemes, and one of the few decentralized \ac{ABE} constructions with full security. Later constructions like RW15~\cite{10.1007/978-3-662-47854-7_19} improve LW11 by allowing large-universe constructions. However, as table \ref{tab:2} showed, LW11 continues to be one of the most deployed schemes.}

% \added{For this experiment, we analyze the LW11 implementation of Rabe, Charm, and GoFE. LW11 is a multi-authority scheme, so the results have a different layout than the GPSW case. In LW11, the \ac{SK} is generated among several authorities, which can each control a variable number of attributes. To perform this operation, each authority must generate its public and private parameters after generating global public parameters. The times for this operation in the case of Charm, Rabe, and GoFE are shown in Figure Y. As with GPSW, GoFE is the least efficient library for this task. And Charm is, again, the most efficient.}

% \added{During regular system operations, authorities work autonomously. Thus, for the same number of attributes, the time required to generate the key is independent of the number of authorities involved in that generation, as seen in the example in \textcolor{red}{FIgureX}. Since they all perform the same operation simultaneously, they all take the same amount of time for the same number of attributes.}

% \added{However, what does affect the authority setup time is the number of attributes that each authority must control. Figure \ref{fig:LW11_AuthSetup_RPI4} shows how this time evolves for a case where there are always five authorities. As the number of attributes controlled by each authority increases, so does time required to generate the key. This implies that if each authority controls a different number of attributes, we can assume that the authority setup will be as slow as the worst case, i.e., the authority controlling more attributes.}

% \begin{figure}[!htbp]
% \centerline{\includegraphics[width=0.75\textwidth]{Figures/LW11_AuthSetup_RPI4.pdf}}
% \caption{LW11 Authority Setup time for 5 authorities in a \ac{RPI4}}
% \label{fig:LW11_AuthSetup_RPI4}
% \end{figure}

% \added{Regarding key generation, we consider the worst-case scenario: that the user requires all attributes of all authorities. This is depicted in Figure \ref{fig:LW11_KeyGen_RPI4}. We can see how the time required for key generation scales linearly with the number of attributes required from each authority. In this case, we can see that Rabe is faster than Charm, despite Charm being faster for authority setup. In fact, Rabe is 162\% faster than Charm (130ms VS 340ms) and 400\% faster than GoFE (130ms VS 650ms).}

% \begin{figure}[!htbp]
% \centerline{\includegraphics[width=0.75\textwidth]{Figures/LW11_KeyGen-RPI4.pdf}}
% \caption{LW11 KeyGen time for 5 authorities in a \ac{RPI4}}
% \label{fig:LW11_KeyGen_RPI4}
% \end{figure}


% \added{When it comes to encryption (Figure \ref{fig:LW11_ENC_RPI4}), Charm regains its place as the faster scheme. We can see that for the best case, Rabe takes 1 second, while Charm takes 240ms. In fact, Charm is capable of encrypting the \ac{PT} always in less than a second, while for the worst-case, Rabe takes almost 2. GoFE, once again, is the least efficient scheme, taking almost 7 seconds for the worst case and 3.6s for the best one.}

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.75\textwidth]{Figures/LW11_ENC_RPI4.pdf}}
% \caption{LW11 Encryption time for 5 authorities in a \ac{RPI4}}
% \label{fig:LW11_ENC_RPI4}
% \end{figure}

% \added{When it comes to decryption (Figure \ref{fig:LW11_DEC_RPI4}), we have similar results to those of encryption, library-performance wise. While Rabe and Charm perform decryption in less than a second, Gofe takes 2,5s for the best case and 5,25s for the worst one. Besides, GoFE has a 4s difference with Rabe and a 5s difference with Charm. As a result, we graph decryption times without GoFE, so the evolution of Charm and Rabe can be appreciated.}

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.75\textwidth]{Figures/LW11_DEC_RPI4.pdf}}
% \caption{LW11 Decryption time for 5 authorities in a \ac{RPI4}}
% \label{fig:LW11_DEC_RPI4}
% \end{figure}

% \added{Figure \ref{fig:LW11_DECSINGOFE_RPI4} shows decryption times of GoFE and Rabe. This figure clearly shows how decryption times are not constant as they seemed in Figure \ref{fig:LW11_DEC_RPI4}. Charm has better times than Rabe, with a difference of 630ms. However, Charm takes 98\% more time from the worst to the best case. Meanwhile, for the same situation, Rabe increased a 41\%. Thus. Charm is faster than Rabe but also increases faster than Rabe. It may be for a very extreme case, for their tendencies to change and Rabe becomes faster than Charm.} \textcolor{red}{SE REPITEN LAS PRUEBAS DE RABE EN LA RPI4, SE GRAFICA Y SE REESCRIBE ESTO}.

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.75\textwidth]{Figures/LW11_DECSINGOFE_RPI4.pdf}}
% \caption{LW11 Decryption time for 5 authorities in a \ac{RPI4}}
% \label{fig:LW11_DECSINGOFE_RPI4}
% \end{figure}


==> recortes.tex <==
De la sección de resultados



\subsubsection{GPSW}\label{Sec:6.1.1}
\added{GPSW~\cite{10.1145/1180405.1180418} was one of the first \ac{ABE} schemes, and falls under the \ac{KP-ABE} approach. The experiments compare the OpenABE and the GoFE implementations. Figure \ref{fig:GPSW_KeyGen-RPI4} shows that key generation times, in ms, are similar in both libraries. GoFe is slower than OpenABE, taking 295ms to generate a key formed by 20 attributes against OpenABE 243 ms. Thus, GoFE takes 21.81\% more time for the same operation.}

\begin{figure}[htbp]
\centerline{\includegraphics[width=0.75\textwidth]{Figures/GPSW_KeyGenRPI4.pdf}}
\caption{GPSW Key Generation times in seconds in a \ac{RPI4}}
\label{fig:GPSW_KeyGen-RPI4}
\end{figure}

\added{When it comes to encryption times, GoFE and OpenABE no longer take a similar amount of times. As Figure \ref{fig:GPSW_Enc-RPI4} shows, although the time continues to grow linear to the number of attributes, GoFE is way less efficient than OpenABE. Even for the case of one attribute, GoFE takes 245ms against OpenABE's 17ms. This difference continues to grow, having a difference of a whole second for the depicted worst-case.}


\begin{figure}[htbp]
\centerline{\includegraphics[width=0.75\textwidth]{Figures/GPSW_Enc_RPI4.pdf}}
\caption{GPSW Encryption times in seconds in a \ac{RPI4}}
\label{fig:GPSW_Enc-RPI4}
\end{figure}

\added{Similar to the case of encryption, decryption also favors OpenABE, as depicted in Figure \ref{fig:GPSW_Dec-RPI4}. Once again, the time required to perform the operations grows linear to the complexity of decryption. This is, of course, the expected growth for this particular scheme. However, the linear growth of GoFE is more pronounced than that of OpenABE. OpenABE starts taking 44ms to decrypt the simplest case against GoFE's 141ms. However, by the end, we can see how for 20 attributes, the difference between OpenaABE and GoFE is 2.4 seconds.}

\begin{figure}[htbp]
\centerline{\includegraphics[width=0.75\textwidth]{Figures/GPSW_DEC_RPI4.pdf}}
\caption{GPSW Decryption times in seconds in a \ac{RPI4}}
\label{fig:GPSW_Dec-RPI4}
\end{figure}

